Resolving Indirect Calls in Binary Code via Cross-Reference Augmented Graph Neural Networks

Binary code analysis is essential in scenarios where source code is unavailable, with extensive applications across various security domains. However, accurately resolving indirect call targets remains a longstanding challenge in maintaining the integrity of static analysis in binary code. This difficulty arises because the operand of a call instruction (e.g., call rax) remains unknown until runtime, resulting in an incomplete inter-procedural control flow graph (CFG). Previous approaches have struggled with low accuracy and limited scalability. To address these limitations, recent work has increasingly turned to machine learning (ML) to enhance analysis. However, this ML-driven approach faces two significant obstacles: low-quality callsite-callee training pairs and inadequate binary code representation, both of which undermine the accuracy of ML models. In this paper, we introduce CupidCall, a novel approach for resolving indirect calls using graph neural networks. Existing ML models in this area often overlook key elements such as data and code cross-references, which are essential for understanding a program's control flow. In contrast, CupidCall augments CFGs with cross-references, preserving rich semantic information. Additionally, we leverage advanced compiler-level type analysis to generate high-quality callsite-callee training pairs, enhancing model precision and reliability. We further design a graph neural model that leverages augmented CFGs and relational graph convolutions for accurate target prediction. Evaluated against real-world binaries from GitHub and the Arch User Repository on x86_64 architecture, CupidCall achieves an F1 score of 95.2%, outperforming state-of-the-art ML-based approaches. These results highlight CupidCall's effectiveness in building precise inter-procedural CFGs and its potential to advance downstream binary analysis and security applications.

==> 5_6_CFI_Evaluation.tex <==
\subsection{Binary-level Control Flow Integrity}


To demonstrate the practical utility of \mytool in security applications, we conducted an experiment to evaluate its effectiveness in simulating a binary-level control flow integrity (CFI) policy. Using Firefox as a case study, we compiled its source code, extracted indirect call targets, and analyzed \mytool's predictions in comparison with LLVM-CFI and Callee.



\vspace*{2pt}
\noindent \textbf{Experimental Setup}
For this application experiment, we compile Firefox into 8
executables, as shown in Column 1 of Table~\ref{table:cfi}.
\mytool is applied directly to these stripped binaries to predict indirect call targets, simulating a binary-level CFI policy. 
Specifically, we retrieve all address-taken (AT) functions in the binary using LLVM and use them as input objects for our prediction model. For each indirect call site in the binary, \mytool calculates the probability of each AT function being the potential callee.
We consider two baselines for our CFI evaluation, LLVM-CFI and Callee. LLVM-CFI is used as a source-level baseline, representing an idealized CFI policy derived from rich compiler-level information, while Callee serves as our baseline for binary-level methods.


To assess the precision of each approach, we employed the average indirect call target (AICT) metric, which measures the average number of targets predicted per indirect call. Lower AICT values indicate greater precision, reducing the attack surface and strengthening the CFI policy.

\vspace*{2pt}
\noindent \textbf{Results and Analysis }
% Our results, presented in Table~\ref{table:cfi}, demonstrates that \mytool consistently achieved AICT values closer to LLVM-CFI compared to Callee. 
% For executables with a large number of icalls, such as ``libnss3.so,'' 
% Callee exhibited substantially higher AICT values, reflecting a greater degree of over-approximation and less alignment with LLVM-CFI’s precision.
% Across the 8 binaries, \mytool reduced the AICT gap with LLVM-CFI by over 44.7\% relative to Callee, indicating that \mytool provides a significantly more precise approximation of source-level CFI policies.
Our results, presented in Table~\ref{table:cfi}, demonstrate that \mytool consistently achieves AICT values closer to LLVM-CFI compared to Callee. For executables with a large number of indirect calls, such as ``libnspr4.so'' and ``libnss3.so,'' Callee exhibited substantially higher AICT values, indicating greater over-approximation and less alignment with LLVM-CFI’s precision. Across the 8 binaries analyzed, \mytool reduced the AICT gap with LLVM-CFI by over 44.7\% relative to Callee, highlighting \mytool’s ability to provide a significantly more precise approximation of source-level CFI policies.




% \begin{itemize}
% 	\item LLVM-CFI: Served as the most precise policy, achieving the lowest AICT values due to its access to source-level type and function information.
% 	\item Callee: Exhibited substantially higher AICT values, reflecting a greater degree of over-approximation and less alignment with LLVM-CFI’s precision.
% 	\item \mytool: Achieved AICT values closely aligned with LLVM-CFI, highlighting its ability to approximate source-level policies despite operating purely on binaries.
	
% \end{itemize}


\begin{table*} [t]
    \centering
    
    \caption{Binary CFI Experiment: \mytool provides a more refined AICT metric compared to Callee and thus closing the gap between LLVM-CFI. ``AT'' in Column 4 is short for Address-Taken functions.}
    \vspace{-2mm}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{ccccccc}
        \topline
        \headcol
        
        \textbf{Binary} & \textbf{\# of Functions} & \textbf{\# of iCalls} & \textbf{\# of AT}  & \thead{\textbf{Callee }\\ \textbf{AICT}} & \thead{\textbf{\mytool }\\ \textbf{AICT}} & \thead{\textbf{LLVM-CFI }\\ \textbf{AICT}} \\
        \midline
        certutil & 1240	& 3 & 408 & \textbf{4.25} & 11 & 5 \\
        \rowcol
        pk12util & 913 & 3 & 345 & \textbf{2.75} & 8.33 & 6.67 \\
        
        signmar & 301 & 1 & 126 & \textbf{2.5} & 3 & 2 \\
        \rowcol
        libfreeblpriv3.so & 4393 & 177 & 1115 & 93.93 & \textbf{45.06} & 29.34 \\
        libnspr4.so & 2008 & 145 & 906 & 181.38 & \textbf{74.79} & 10.61 \\
        \rowcol
        libmozsqlite3.so & 7110 & 907 & 905 & 202.78 & \textbf{139.76} & 33.12 \\
        libnss3.so & 5682 & 383 & 2548 & 330.88 & \textbf{204.32} & 15.27 \\
        \rowcol
        libssl3.so & 3482 & 373	& 1410 & 82.17 & \textbf{65.96} & 19.52 \\
        \bottomline
    \end{tabular}
    
    \label{table:cfi}
}
\vspace{-5mm}
\end{table*}
